Bistable Probabilities: A Unified Framework for Studying Rationality and Irrationality in Classical and Quantum Games

This article presents a unified probabilistic framework that allows both rational and irrational decision making to be theoretically investigated and simulated in classical and quantum games. Rational choice theory is a basic component of game theoretic models, which assumes that a decision maker chooses the best action according to their preferences. In this article, we define irrationality as a deviation from a rational choice. Bistable probabilities are proposed as a principled and straight forward means for modeling irrational decision making in games. Bistable variants of classical and quantum Prisoner's Dilemma, Stag Hunt and Chicken are analyzed in order to assess the effect of irrationality on agent utility and Nash equilibria. It was found that up to three Nash equilibria exist for all three classical bistable games and maximal utility was attained when agents were rational. Up to three Nash equilibria exist for all three quantum bistable games, however, utility was shown to increase according to higher levels of agent irrationality.

==> references1.tex <==
@PREAMBLE{
 "\providecommand{\noopsort}[1]{}" 
 # "\providecommand{\singleletter}[1]{#1}%" 
}

@article{meyer1999quantum,
  title={Quantum strategies},
  author={Meyer, David A},
  journal={Physical Review Letters},
  volume={82},
  number={5},
  pages={1052},
  year={1999},
  publisher={APS}
}



@article{eisert2000quantum,
  title={Quantum games},
  author={Eisert, Jens and Wilkens, Martin},
  journal={Journal of Modern Optics},
  volume={47},
  number={14-15},
  pages={2543--2556},
  year={2000},
  publisher={Taylor \& Francis}
}

@article{zurek2000einselection,
  title={Einselection and decoherence from an information theory perspective},
  author={Zurek, Wojciech H},
  journal={Annalen der Physik},
  volume={9},
  number={11-12},
  pages={855--864},
  year={2000},
  publisher={Wiley Online Library}
}

@article{girolami2014quantum,
  title={Quantum discord determines the interferometric power of quantum states},
  author={Girolami, Davide and Souza, Alexandre M and Giovannetti, Vittorio and Tufarelli, Tommaso and Filgueiras, Jefferson G and Sarthour, Roberto S and Soares-Pinto, Diogo O and Oliveira, Ivan S and Adesso, Gerardo},
  journal={Physical Review Letters},
  volume={112},
  number={21},
  pages={210401},
  year={2014},
  publisher={APS}
}

@article{dehdashti2016stability,
  title={Stability of two interacting entangled spins interacting with a thermal environment.},
  author={Dehdashti, Shahram and Harouni, MB and Harsij, Z and Shen, J and Wang, H and Xu, Z and Mirza, B and Chen, H},
  journal={Quantum Information \& Computation},
  volume={16},
  number={15\&16},
  pages={1365--1378},
  year={2016}
}

@incollection{kochen1975problem,
  title={The problem of hidden variables in quantum mechanics},
  author={Kochen, Simon and Specker, Ernst P},
  booktitle={The logico-algebraic approach to quantum mechanics},
  pages={293--328},
  year={1975},
  publisher={Springer}
}

@article{liang2011specker,
  title={Specker’s parable of the overprotective seer: A road to contextuality, nonlocality and complementarity},
  author={Liang, Yeong-Cherng and Spekkens, Robert W and Wiseman, Howard M},
  journal={Physics Reports},
  volume={506},
  number={1-2},
  pages={1--39},
  year={2011},
  publisher={Elsevier}
}

@article{pitowsky1994george,
  title={George Boole's ‘conditions of possible experience’and the quantum puzzle},
  author={Pitowsky, Itamar},
  journal={The British Journal for the Philosophy of Science},
  volume={45},
  number={1},
  pages={95--125},
  year={1994},
  publisher={Oxford University Press}
}

@article{goh2018geometry,
  title={Geometry of the set of quantum correlations},
  author={Goh, Koon Tong and Kaniewski, J{\k{e}}drzej and Wolfe, Elie and V{\'e}rtesi, Tam{\'a}s and Wu, Xingyao and Cai, Yu and Liang, Yeong-Cherng and Scarani, Valerio},
  journal={Physical Review A},
  volume={97},
  number={2},
  pages={022104},
  year={2018},
  publisher={APS}
}

@article{vourdas2019probabilistic,
  title={Probabilistic inequalities and measurements in bipartite systems},
  author={Vourdas, Apostol},
  journal={Journal of Physics A: Mathematical and Theoretical},
  year={2019},
  publisher={IOP Publishing}
}

@book{busemeyer2012quantum,
  title={Quantum models of cognition and decision},
  author={Busemeyer, Jerome R and Bruza, Peter D},
  year={2012},
  publisher={Cambridge University Press}
}

@article{big2018challenging,
  title={Challenging local realism with human choices.},
  author={BIG Bell Test Collaboration and others},
  journal={Nature},
  volume={557},
  number={7704},
  pages={212},
  year={2018}
}

@article{allen2017quantum,
  title={Quantum common causes and quantum causal models},
  author={Allen, John-Mark A and Barrett, Jonathan and Horsman, Dominic C and Lee, Ciar{\'a}n M and Spekkens, Robert W},
  journal={Physical Review X},
  volume={7},
  number={3},
  pages={031021},
  year={2017},
  publisher={APS}
}

@article{brunner2013connection,
  title={Connection between Bell nonlocality and Bayesian game theory},
  author={Brunner, Nicolas and Linden, Noah},
  journal={Nature communications},
  volume={4},
  pages={2057},
  year={2013},
  publisher={Nature Publishing Group}
}

@article{iqbal2016equivalence,
  title={On the equivalence between non-factorizable mixed-strategy classical games and quantum games},
  author={Iqbal, Azhar and Chappell, James M and Abbott, Derek},
  journal={Royal Society open science},
  volume={3},
  number={1},
  pages={150477},
  year={2016},
  publisher={The Royal Society Publishing}
}

@article{alonso2019collective,
  title={On collective quantum games},
  author={Alonso-Sanz, Ram{\'o}n},
  journal={Quantum Information Processing},
  volume={18},
  number={3},
  pages={64},
  year={2019},
  publisher={Springer}
}

@article{hoffman2014objects,
  title={Objects of consciousness},
  author={Hoffman, Donald D and Prakash, Chetan},
  journal={Frontiers in Psychology},
  volume={5},
  pages={577},
  year={2014},
  publisher={Frontiers}
}


@article{costello2014surprisingly,
  title={Surprisingly rational: Probability theory plus noise explains biases in judgment.},
  author={Costello, Fintan and Watts, Paul},
  journal={Psychological review},
  volume={121},
  number={3},
  pages={463},
  year={2014},
  publisher={American Psychological Association}
}

@article{costello2016people,
  title={People’s conditional probability judgments follow probability theory (plus noise)},
  author={Costello, Fintan and Watts, Paul},
  journal={Cognitive psychology},
  volume={89},
  pages={106--133},
  year={2016},
  publisher={Elsevier}
}

@article{costello2017explaining,
  title={Explaining high conjunction fallacy rates: The probability theory plus noise account},
  author={Costello, Fintan and Watts, Paul},
  journal={Journal of Behavioral Decision Making},
  volume={30},
  number={2},
  pages={304--321},
  year={2017},
  publisher={Wiley Online Library}
}

@article{costello2018surprising,
  title={Surprising rationality in probability judgment: Assessing two competing models},
  author={Costello, Fintan and Watts, Paul and Fisher, Christopher},
  journal={Cognition},
  volume={170},
  pages={280--297},
  year={2018},
  publisher={Elsevier}
}

@article{costello2019rationality,
  title={The rationality of illusory correlation.},
  author={Costello, Fintan and Watts, Paul},
  journal={Psychological review},
  volume={126},
  number={3},
  pages={437},
  year={2019},
  publisher={American Psychological Association}
}

@article{spekkens2007evidence,
  title={Evidence for the epistemic view of quantum states: A toy theory},
  author={Spekkens, Robert W},
  journal={Physical Review A},
  volume={75},
  number={3},
  pages={032110},
  year={2007},
  publisher={APS}
}

@article{press2012iterated,
  title={Iterated Prisoner’s Dilemma contains strategies that dominate any evolutionary opponent},
  author={Press, William H and Dyson, Freeman J},
  journal={Proceedings of the National Academy of Sciences},
  volume={109},
  number={26},
  pages={10409--10413},
  year={2012},
  publisher={National Acad Sciences}
}

@article{gold2007neural,
  title={The neural basis of decision making},
  author={Gold, Joshua I and Shadlen, Michael N},
  journal={Annu. Rev. Neurosci.},
  volume={30},
  pages={535--574},
  year={2007},
  publisher={Annual Reviews}
}

@article{fleming2016decision,
  title={Decision Making: Changing our minds about changes of mind},
  author={Fleming, Stephen M},
  journal={Elife},
  volume={5},
  pages={e14790},
  year={2016},
  publisher={eLife Sciences Publications Limited}
}

@article{resulaj2009changes,
  title={Changes of mind in decision-making},
  author={Resulaj, Arbora and Kiani, Roozbeh and Wolpert, Daniel M and Shadlen, Michael N},
  journal={Nature},
  volume={461},
  number={7261},
  pages={263},
  year={2009},
  publisher={Nature Publishing Group}
}

@article{cavanagh2014frontal,
  title={Frontal theta as a mechanism for cognitive control},
  author={Cavanagh, James F and Frank, Michael J},
  journal={Trends in cognitive sciences},
  volume={18},
  number={8},
  pages={414--421},
  year={2014},
  publisher={Elsevier}
}

@article{atiya2019neural,
  title={A neural circuit model of decision uncertainty and change-of-mind},
  author={Atiya, Nadim AA and Ra{\~n}{\'o}, I{\~n}aki and Prasad, Girijesh and Wong-Lin, KongFatt},
  journal={Nature communications},
  volume={10},
  number={1},
  pages={2287},
  year={2019},
  publisher={Nature Publishing Group}
}


@article{becks2019extortion,
  title={Extortion strategies resist disciplining when higher competitiveness is rewarded with extra gain},
  author={Becks, Lutz and Milinski, Manfred},
  journal={Nature communications},
  volume={10},
  number={1},
  pages={783},
  year={2019},
  publisher={Nature Publishing Group}
}

@article{fell2019experimental,
  title={An Experimental Protocol to Derive and Validate a Quantum Model of Decision-Making},
  author={Fell, Lauren and Dehdashti, Shahram and Bruza, Peter and Moreira, Catarina},
  journal={arXiv preprint arXiv:1908.07935},
  year={2019}
}
@article{busch1986unsharp,
  title={Unsharp reality and joint measurements for spin observables},
  author={Busch, Paul},
  journal={Physical Review D},
  volume={33},
  number={8},
  pages={2253},
  year={1986},
  publisher={APS}
}


@book{simon:1957,
	Author = {Simon, H.A.},
	Date-Added = {2016-10-20 23:39:44 +0000},
	Date-Modified = {2016-10-20 23:40:47 +0000},
	Publisher = {Wiley},
	Title = {Models of Man: Social and Rational},
	Year = {1957}}
	
	
@book{Gigenrenzer:Todd:1999,
	Author = {Gigerenzer, G. and Todd, P.M.},
	Date-Added = {2019-08-19 08:37:21 +1000},
	Date-Modified = {2019-08-19 08:38:54 +1000},
	Publisher = {Oxford University Press},
	Title = {Simple Heuristics That Make Us Smart},
	Year = {1999}}


@article{baranowski:summers:72,
	Author = {Baranowski, T.A. and Summers, D.A.},
	Date-Added = {2019-08-19 08:45:39 +1000},
	Date-Modified = {2019-08-19 08:48:12 +1000},
	Journal = {Journal of Personality and Social Psychology},
	Number = {1},
	Pages = {35-40},
	Title = {Perception of response alternatives in a prisoner's dilemma game},
	Volume = {21},
	Year = {1972}}


@article{chater:vlaev:grinberg:2008,
	Author = {Chater, N. and Vlaev, I. and Grinberg, M.},
	Date-Added = {2019-08-19 08:50:07 +1000},
	Date-Modified = {2019-08-19 08:52:46 +1000},
	Journal = {Journal of Experimental Psychology: General},
	Number = {3},
	Pages = {403-421},
	Title = {A New Consequence of Simpson's Paradox: Stable Cooperation in One- Shot Prisoner's Dilemma From Populations of Individualistic Learners},
	Volume = {137},
	Year = {2008}}


@article{pothos:busemeyer:2011,
	Author = {Pothos, E.M. and Perry, G. and Corr, P.J. and Mathew, M.R. and Busemeyer, J.},
	Date-Added = {2019-08-19 08:55:55 +1000},
	Date-Modified = {2019-08-19 08:58:36 +1000},
	Journal = {Personality and Individual Differences},
	Pages = {210-215},
	Title = {Understanding cooperation in the Prisoner's Dilemma game},
	Volume = {51},
	Year = {2011}}


@article{khadjavi:lang:2013,
	Author = {Khadjavi, M. and Lange, A.},
	Date-Added = {2019-08-19 09:00:46 +1000},
	Date-Modified = {2019-08-19 09:02:25 +1000},
	Journal = {Journal of Economic Behavior \& Organization},
	Pages = {163-175},
	Title = {Prisoners and their dilemma},
	Volume = {92},
	Year = {2013}}


@article{bruza:wang:busemeyer:2015,
	Author = {Peter D. Bruza and Zheng Wang and Jerome R. Busemeyer},
	Date-Added = {2015-07-06 03:18:25 +0000},
	Date-Modified = {2016-10-21 04:40:28 +0000},
	Journal = {Trends in Cognitive Sciences},
	Keywords = {human judgment},
	Number = {7},
	Pages = {383 - 393},
	Title = {Quantum cognition: a new theoretical approach to psychology},
	Volume = {19},
	Year = {2015}
}


@article{busemeyer:pothos:franco:trueblood:2011,
	Author = {Busemeyer, J. and Pothos, E.M. and Franco, R. and Trueblood, J.S},
	Date-Added = {2011-05-11 14:10:13 +1000},
	Date-Modified = {2011-05-11 14:12:35 +1000},
	Journal = {Psychological Review},
	Number = {2},
	Pages = {193-218},
	Title = {A quantum theoretical explanation for probability judgment errors},
	Volume = {118},
	Year = {2011}}

}

@incollection{gladwin:figner:2015,
                Author = {Gladwin, T.E. and Figner, B.},
                Booktitle = {Neuroeconomics, Judgment and Decision Making},
                Chapter = {8},
                Editor = {Wilhelms, E.A. and Reyna, V.F.},
                Pages = {157-180},
                Publisher = {Psychology Press},
                Series = {Frontiers of Cognitive Psychology},
                Title = {{``Hot"} Cognition and Dual Systems: Introduction, Criticisms and Ways forward},
                Year = {2015}}



@book{kahneman2011thinking,
  title={Thinking, fast and slow},
  author={Kahneman, Daniel},
  year={2011},
  publisher={Macmillan}
}

@article{evans2003two,
  title={In two minds: dual-process accounts of reasoning},
  author={Evans, Jonathan St BT},
  journal={Trends in cognitive sciences},
  volume={7},
  number={10},
  pages={454--459},
  year={2003},
  publisher={Elsevier}
}

@article{capraro2014heuristics,
  title={Heuristics guide the implementation of social preferences in one-shot Prisoner's Dilemma experiments},
  author={Capraro, Valerio and Jordan, Jillian J and Rand, David G},
  journal={Scientific reports},
  volume={4},
  pages={6790},
  year={2014},
  publisher={Nature Publishing Group}
}

@article{dehdashti2020irrationality,
  title={On the Irrationality of Being in Two Minds},
  author={Dehdashti, Shahram and Fell, Lauren and Bruza, Peter},
  journal={Entropy},
  volume={22},
  number={2},
  pages={174},
  year={2020},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@article{makowski2014cut,
  title={When I cut, you choose method implies intransitivity},
  author={Makowski, Marcin and Piotrowski, Edward W},
  journal={Physica A: Statistical Mechanics and its Applications},
  volume={415},
  pages={189--193},
  year={2014},
  publisher={Elsevier}
}

@article{makowski2011transitivity,
  title={Transitivity of an entangled choice},
  author={Makowski, Marcin and Piotrowski, Edward W},
  journal={Journal of Physics A: Mathematical and Theoretical},
  volume={44},
  number={7},
  pages={075301},
  year={2011},
  publisher={IOP Publishing}
}

@article{makowski2015transitive,
  title={Do transitive preferences always result in indifferent divisions?},
  author={Makowski, Marcin and Piotrowski, Edward W and S{\l}adkowski, Jan},
  journal={Entropy},
  volume={17},
  number={3},
  pages={968--983},
  year={2015},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@article{makowski2017profit,
  title={Profit intensity and cases of non-compliance with the law of demand/supply},
  author={Makowski, Marcin and Piotrowski, Edward W and S{\l}adkowski, Jan and Syska, Jacek},
  journal={Physica A: Statistical Mechanics and its Applications},
  volume={473},
  pages={53--59},
  year={2017},
  publisher={Elsevier}
}

@article{uprety2020quantum,
  title={Quantum-like structure in multidimensional relevance judgements},
  author={Uprety, Sagar and Tiwari, Prayag and Dehdashti, Shahram and Fell, Lauren and Song, Dawei and Bruza, Peter and Melucci, Massimo},
  journal={arXiv preprint arXiv:2001.07075},
  year={2020}
}

@book{buchak:2013,
	Author = {Buchak, L.},
	Publisher = {Oxford University Press},
	Title = {Risk and Rationality},
	Year = {2013}}


@article{vlaev:2018,
	Author = {Vlaev, I.},
	Journal = {Brain Sciences},
	Number = {8},
	Title = {Local choices: Rationality and the contextuality of decision-making},
	Volume = {8},
	Year = {2018}}


@article{chater:oaksford:2000,
	Author = {Chater, N. and Oaksford, M.},
	Journal = {Synthese},
	Number = {1},
	Pages = {93---131},
	Title = {The rational analysis of mind and behavior},
	Volume = {122},
	Year = {2000}}


@article{howes:lewis:vera:2009,
	Author = {Howes, A. and Lewis, R.L. and Vera, A.},
	Journal = {Psychological Review},
	Number = {4},
	Pages = {717--751},
	Title = {Rational adaptation under task and processing constraints: Implications for testing theories of cognition and action},
	Volume = {116},
	Year = {2009}}


@incollection{bicchieri:2004,
	Author = {Bicchieri, C.},
	Booktitle = {The Oxford Handbook of Rationality},
	Chapter = {10},
	Editor = {Mele, A.R. and Rawling, P.},
	Publisher = {Oxford University Press},
	Title = {Rationality and Game Theory},
	Year = {2004}}

@article{lieberman2005evolutionary,
  title={Evolutionary dynamics on graphs},
  author={Lieberman, Erez and Hauert, Christoph and Nowak, Martin A},
  journal={Nature},
  volume={433},
  number={7023},
  pages={312–316},
  year={2005},
  publisher={Nature Publishing Group}
}


@article{nowak2006five,
  title={Five rules for the evolution of cooperation},
  author={Nowak, Martin A},
  journal={science},
  volume={314},
  number={5805},
  pages={1560–1563},
  year={2006},
  publisher={American Association for the Advancement of Science}
}


@article{perc2017statistical,
  title={Statistical physics of human cooperation},
  author={Perc, Matja{\v{z}} and Jordan, Jillian J and Rand, David G and Wang, Zhen and Boccaletti, Stefano and Szolnoki, Attila},
  journal={Physics Reports},
  volume={687},
  pages={1–51},
  year={2017},
  publisher={Elsevier}
}


@article{eisert1999quantum,
  title={Quantum games and quantum strategies},
  author={Eisert, Jens and Wilkens, Martin and Lewenstein, Maciej},
  journal={Physical Review Letters},
  volume={83},
  number={15},
  pages={3077},
  year={1999},
  publisher={APS}
}

@article{iqbal2002quantum,
  title={Quantum cooperative games},
  author={Iqbal, A and Toor, AH},
  journal={Physics Letters A},
  volume={293},
  number={3-4},
  pages={103–108},
  year={2002},
  publisher={Elsevier}
}

@article{mcconnell2015entanglement,
  title={Entanglement with negative Wigner function of almost 3,000 atoms heralded by one photon},
  author={McConnell, Robert and Zhang, Hao and Hu, Jiazhong and {\’C}uk, Senka and Vuleti{\’c}, Vladan},
  journal={Nature},
  volume={519},
  number={7544},
  pages={439–442},
  year={2015},
  publisher={Nature Publishing Group}
}

@article{evans2007resolution,
  title={On the resolution of conflict in dual process theories of reasoning},
  author={Evans, Jonathan St BT},
  journal={Thinking \& Reasoning},
  volume={13},
  number={4},
  pages={321--339},
  year={2007},
  publisher={Taylor \& Francis}
}

@article{rand2016social,
  title={Social heuristics and social roles: Intuition favors altruism for women but not for men.},
  author={Rand, David G and Brescoll, Victoria L and Everett, Jim AC and Capraro, Valerio and Barcelo, H{\'e}l{\`e}ne},
  journal={Journal of Experimental Psychology: General},
  volume={145},
  number={4},
  pages={389},
  year={2016},
  publisher={American Psychological Association}
}


@article{balliet2009social,
  title={Social value orientation and cooperation in social dilemmas: A meta-analysis},
  author={Balliet, Daniel and Parks, Craig and Joireman, Jeff},
  journal={Group Processes \& Intergroup Relations},
  volume={12},
  number={4},
  pages={533--547},
  year={2009},
  publisher={Sage Publications Sage UK: London, England}
}

@article{rand2013human,
  title={Human cooperation},
  author={Rand, David G and Nowak, Martin A},
  journal={Trends in cognitive sciences},
  volume={17},
  number={8},
  pages={413--425},
  year={2013},
  publisher={Elsevier}
}

@article{axelrod1981evolution,
  title={The evolution of cooperation},
  author={Axelrod, Robert and Hamilton, William Donald},
  journal={science},
  volume={211},
  number={4489},
  pages={1390--1396},
  year={1981},
  publisher={American Association for the Advancement of Science}
}

@article{dana2007exploiting,
  title={Exploiting moral wiggle room: experiments demonstrating an illusory preference for fairness},
  author={Dana, Jason and Weber, Roberto A and Kuang, Jason Xi},
  journal={Economic Theory},
  volume={33},
  number={1},
  pages={67--80},
  year={2007},
  publisher={Springer}
}

@article{moisan2018not,
  title={Not all Prisoner’s Dilemma games are equal: Incentives, social preferences, and cooperation.},
  author={Moisan, Fr{\'e}d{\'e}ric and ten Brincke, Robert and Murphy, Ryan O and Gonzalez, Cleotilde},
  journal={Decision},
  volume={5},
  number={4},
  pages={306},
  year={2018},
  publisher={Educational Publishing Foundation}
}

@article{rilling2002neural,
  title={A neural basis for social cooperation},
  author={Rilling, James K and Gutman, David A and Zeh, Thorsten R and Pagnoni, Giuseppe and Berns, Gregory S and Kilts, Clinton D},
  journal={Neuron},
  volume={35},
  number={2},
  pages={395--405},
  year={2002},
  publisher={Elsevier}
}

@article{kahneman1997back,
  title={Back to Bentham? Explorations of experienced utility},
  author={Kahneman, Daniel and Wakker, Peter P and Sarin, Rakesh},
  journal={The quarterly journal of economics},
  volume={112},
  number={2},
  pages={375--406},
  year={1997},
  publisher={MIT Press}
}

@article{kahneman2006anomalies,
  title={Anomalies: Utility maximization and experienced utility},
  author={Kahneman, Daniel and Thaler, Richard H},
  journal={Journal of economic perspectives},
  volume={20},
  number={1},
  pages={221--234},
  year={2006}
}

@article{rand2014social,
  title={Social heuristics shape intuitive cooperation},
  author={Rand, David G and Peysakhovich, Alexander and Kraft-Todd, Gordon T and Newman, George E and Wurzbacher, Owen and Nowak, Martin A and Greene, Joshua D},
  journal={Nature communications},
  volume={5},
  number={1},
  pages={1--12},
  year={2014},
  publisher={Nature Publishing Group}
}

@article{capraro2019dual,
  title={The dual-process approach to human sociality: A review},
  author={Capraro, Valerio},
  journal={Available at SSRN 3409146},
  year={2019}
}

@article{engel2016risk,
  title={When is the risk of cooperation worth taking? The prisoner’s dilemma as a game of multiple motives},
  author={Engel, Christoph and Zhurakhovska, Lilia},
  journal={Applied Economics Letters},
  volume={23},
  number={16},
  pages={1157--1161},
  year={2016},
  publisher={Taylor \& Francis}
}

@article{moreira_fell_dehdashti_bruza_wichert_2020, title={Towards a quantum-like cognitive architecture for decision-making}, volume={43}, DOI={10.1017/S0140525X19001687}, journal={Behavioral and Brain Sciences}, publisher={Cambridge University Press}, author={Moreira, Catarina and Fell, Lauren and Dehdashti, Shahram and Bruza, Peter and Wichert, Andreas}, year={2020}, pages={e17}}

@article{rand2012spontaneous,
  title={Spontaneous giving and calculated greed},
  author={Rand, David G and Greene, Joshua D and Nowak, Martin A},
  journal={Nature},
  volume={489},
  number={7416},
  pages={427--430},
  year={2012},
  publisher={Nature Publishing Group}
}

@article{isler2018intuition,
  title={Is intuition really cooperative? Improved tests support the social heuristics hypothesis},
  author={Isler, Ozan and Maule, John and Starmer, Chris},
  journal={PloS one},
  volume={13},
  number={1},
  year={2018},
  publisher={Public Library of Science}
}

@article{cone2014time,
  title={Time pressure increases cooperation in competitively framed social dilemmas},
  author={Cone, Jeremy and Rand, David G},
  journal={PLoS one},
  volume={9},
  number={12},
  year={2014},
  publisher={Public Library of Science}
}



@article{Hodgson:2012,
	Author = {Hodgson, G.M.},
	Journal = {Economic Thought},
	Number = {1},
	Pages = {94-108},
	Title = {On the limits of rational choice theory},
	Volume = {1},
	Year = {2012}}

